A behavioural transformer for effective collaboration between a robot and a non-stationary human

A key challenge in human-robot collaboration is the non-stationarity created by humans due to changes in their behaviour. This alters environmental transitions and hinders human-robot collaboration. We propose a principled meta-learning framework to explore how robots could better predict human behaviour, and thereby deal with issues of non-stationarity. On the basis of this framework, we developed Behaviour-Transform (BeTrans). BeTrans is a conditional transformer that enables a robot agent to adapt quickly to new human agents with non-stationary behaviours, due to its notable performance with sequential data. We trained BeTrans on simulated human agents with different systematic biases in collaborative settings. We used an original customisable environment to show that BeTrans effectively collaborates with simulated human agents and adapts faster to non-stationary simulated human agents than SOTA techniques.

==> sections/problem_statement/transition_model.tex <==
In our setting, the human updates its latent strategy at every time step according to the human's history dependent process $\rho$. 

\begin{figure}[H]
\centering
\includegraphics[width=0.33\paperwidth]{images/transition_model.PNG}
\caption{Transition model}
\label{fig:transition model}
\end{figure}

\begin{equation}
\begin{split}
    p_\pi (\tau) = d_0 (s_0) \prod_{t=0}^H \pi (a_{R,t} | s_{0 : t}) T(s_{t+1} | s_t, a_{R,t}, z_t) \\ \rho (z_t | s_t, a_{R,t}, z_{0 : t-1})
\end{split}
\end{equation}

==> sections/proposed_approach/data.tex <==
A long-time series can be difficult to feed into a transformer. Therefore, the data were split into several smaller windows of 25 time steps. 

% \begin{figure}
% \centering
% \includegraphics[width=0.4\paperwidth]{images/dataset_split.png}
% \caption{Transformer model}
% \label{fig:transformer model}
% \end{figure}

==> sections/related_work/MARL.tex <==
Several multi-agent reinforcement learning (MARL) techniques have been suggested for dealing with non-stationarity \cite{albrecht_autonomous_2018}. Effective MARL approaches have adopted a centralised framework to enable multiple agents to coordinate their behaviour together and collaborate effectively. However, in pHRC scenarios, the training needs to be decentralised as it is not possible to control both of the agents – only the reinforcement learning robot agent. Therefore, the human agent needs to be created as part of the environment and a separate model of the human is required to predict and influence its behaviour.  

==> sections/related_work/experiment.tex <==
An advantage of our approach is that it allows adaption to different humans whose behaviour changes over time.\\

We compare our approach against three methods: 
\begin{itemize}
    \item \textbf{Oracle:} This approach knows the ground truth latent state of the human and provides and upper bound on the performance of our method. 
    \item \textbf{SAC:} This approaches does not explicitly model the dynamics of a human
    \item \textbf{LILI:} This approach learns the dynamics of a human and provides a baseline to compare our approach against.
    \item \textbf{MMBT}: Our approach that adapts to unseen human's with changing behaviour.
\end{itemize}

==> sections/related_work/human_model.tex <==
Reinforcement learning requires large amounts of data to be generated for the robot to adapt to non-stationary humans. Synthetic humans offer one way of dealing with this issue. There have been several approaches adopted to creating synthetic human models for training robots. One way is to create the synthetic human from programming rules. \theo{citation needed }
This allows synthetic humans to be created easily, but the simulation typically does not match real human behaviour. An alternative approach uses supervised methods to learn a policy capable of mapping human actions to what is observed (imitation learning). This circumvents assumptions about human behaviour, but requires large amount of data, has distribution shift, and struggles to generalise. \theo{citations are needed in all the above}
Another technique is to assume that the human acts with respect to a reward, and to use that reward to predict the behaviour (or vice versa) \cite{yang_optimal_2022,reddy_where_2019,laidlaw_boltzmann_2022}.
\theo{citate also Daniel's latest paper}
There are several assumptions that are made when mapping from behaviour to reward. The first is to assume that humans act perfectly rationally. The second is to assume that humans act optimally but with added noise. This gives the assumption of Boltzmann rationality which is the prevalent approach, but ignores a range of systematic biases \cite{chan_human_2021}.\\

In this paper, synthetic humans will be generated with different systematic biases for the robot to train with. The focus is on developing a robot policy that can collaborate with humans with different dynamics.

==> sections/related_work/influencing.tex <==
To successfully complete tasks in pHRC, it may be critical for the robot to influence the human. There are two purposes of this. The first is to influence the human to limit the possibilities of their behaviour so that the robot can make accurate predictions. The second is to influence toward more desirable limiting behaviours so that the robot can maximise its reward. The robot can shape the human’s policy updates (changes in behaviour). We focus on leverage the dependencies of the robot’s actions on the human’s behaviour to shape the convergence process for repeated interactions. Related to our approach is LILI, SILI and RILI. These methods learn a high-level latent strategy for the human and condition a single-agent RL policy on this learned latent strategy. The method leverages recurring neural network (RNNs) or feed-forward neural networks (MLPs) as part of the encoder and decoder blocks to learn the latent strategy.

==> sections/related_work/introduction.tex <==
A key challenge in enabling robots to learn effective policies in pHRC scenarios relates to the human changing their behaviour over time (non-stationarity in reinforcement learning). There has been work in multiagent reinforcement learning (MARL) to tackle non-stationarity, but the approaches use a centralised framework which is not possible in physical human-robot collaboration settings when there is a human that needs to be treated as part of the environment and modelled separately. One way to model a human is by assuming that they are governed by a latent state. This allows the non-stationarity problem to be tackled through the paradigm of zero-shot meta learning, where each behaviour (latent state) is treated as a separate task and the robot needs to instantly adapt to new tasks.  Different methods exist to predict the current human behaviour, or latent state, from history information. \theo{citations are needed in all the above, roughly 1 per statement, hence around 4-5 for the text above}


\theo{the following has a separate main message than the above, hence I separated.}
Transformers have been shown to learn effectively the semantic relationships between sequential elements. Transformers, therefore, could provide a  promising approach for predicting future behaviour. However, transformers, alongside reinforcement learning methods, require significant amounts of data for training. One solution to address the issue of generating training data is to use synthetic humans. There are several methods available to create synthetic humans capable of mimicking real human behaviour and thereby allowing data to be generated for the purpose of training the robot. These issues are addressed in turn below. \theo{citations are needed in all the above, roughly 1 per statement, hence around 2-3 for the text above}


\subsection{What LILI cannot do}
\begin{itemize}
    \item Cannot handle noise in observations (only perfect observations, none stochastic observation model)
    \item Performs poor with long episode lengths ($\geq$ 10 timesteps)
    \item Performs poor with respect to longer histories (related to the number of episodes)
    \item Requires a fixed number of timesteps for the ball to travel between paddles
    \item Do not assume when the human changes behaviour (it can be at any timestep)
    \item Can take variable length inputs to predict the human behaviour (which will help in ad hoc coordination)
    
\end{itemize}

==> sections/related_work/learning_latent_strategies.tex <==
Modelling the human by learning a low-level policy may be computationally inefficient. There may be an implicit structure in the human’s policy space that can be captured in a lower dimension. Prior work has captured this low-dimensional term as a latent strategy. This can be depicted as the high level strategy of the human, or their goal. Previous work has treated different latent variables as different tasks, which the robot’s policy can distinguish between. Each task represents a fundamentally different human behaviour. LILI, SILI and RILI \cite{wang_uencing_nodate, parekh_rili_2022, xie_learning_2020} learn a high-level latent strategy for the human and condition a single-agent RL policy on this strategy. LILI, SILI and RILI lever recurring neural network (RNNs) or feed-forward neural networks (MLPs) within encoder and decoder blocks to learn the latent strategy. \theo{here mention MLPs and RNNs drawbacks}


==> sections/related_work/meta_RL.tex <==
Meta-RL provides a paradigm for leveraging latent strategies to deal with non-stationarity. Meta-RL ("learning to learn") utilises a set of tasks with a common form during a training phase to enable quick adaption to similar but new tasks unseen during training. One approach - which will be adopted in this paper - is to consider meta-RL as an expansion of multi-task RL where the task information must be inferred. Meta-RL refers to learning a multi-task robot policy  $\pi_{\theta}$ and inferring the task $z$. Meta-RL consists of two settings for adapting to new tasks. First, 'few-shot' (episodic) adaptation where the agent is allowed to collect data for a few episodes. Second, 'zero-shot' adaptation where the agent may encounter a new task at every timestep and react immediately. The zero-shot adaptation setting is thus relevant to the non-stationarity issue. In this paper we use the zero-shot meta-learning approach to enable the robot to deal with non-stationarity. \theo{not sure if it does zero-shot learning}


==> sections/related_work/reinforcement_learning.tex <==
Reinforcement learning (RL) techniques enable robots to learn optimum decisions in stationary environments.  However, the human can be considered as part of the environment in pHRC scenarios, so the environmental dynamics change when human behaviour alters ("non-stationarity"). Thus, traditional RL methods yield sub-optimal decisions in pHRC scenarios. \theo{citation  is needed in all the above}


==> sections/related_work/transformers.tex <==
Transformers offer a promising approach for predicting future behaviour given sequential history information \cite{vaswani_attention_2017}. These models have shown strong performance in capturing long-range dependencies, and have generally improved performance over recurring neural network models (RNNs) for processing sequential data. Our approach uses a transformer due to its ability to identify sequential correlations. 
